A Measurement Study of the Impact of Adjacent Channel Interference between C-band and CBRS

The 3.7 - 3.98 GHz frequency band (also known as C-band) was recently allocated in the US for the deployment of 5G cellular services. Prior to this, the lower adjacent band, 3.55 - 3.7 GHz, had been allocated to Citizens Broadband Radio Service (CBRS), where the entire 150 MHz can be used for free by Tier 3 General Authorized Access (GAA) users, but access to the spectrum needs to be authorized by the Spectrum Access System (SAS). GAA users are allowed on a channel only when there are no Tier 1 Incumbents (Navy radars) or Tier 2 Priority Access License (PAL) users in the area. However, since there are no guard bands between GAA and C-band, and both systems employ Time Division Duplexing (TDD) where the uplink/downlink configurations are not synchronized, adjacent channel interference can potentially reduce the performance of both systems. In this paper, we quantify the effect of this mutual interference by performing experiments with a real-world deployment. We observe significant downlink throughput reductions on both systems when two devices are in close proximity to each other, and one is transmitting uplink while the other is transmitting downlink: 60% for 4G CBRS and 43% for 5G C-band. We believe that this is the first paper to demonstrate this in a real deployment. This throughput degradation was reduced when the CBSD changed its channel and operated 20 MHz away from C-band, essentially creating a guard band between the channels. We also demonstrate the improvement in latency under adjacent channel interference by implementing MicroSlicing at the CBSD. Our results indicate that addressing adjacent channel interference due to the lack of guard bands and TDD configuration mismatch is crucial to improving the performance of both CBRS and C-band systems.

==> sections/04.5_deployment.tex <==
\section{5G Deployment Details}
\label{sec:deployment}

Preliminary measurements showed a number of different 4G LTE and 5G NR signals that were received inside the building from deployed AT\&T, T-Mobile, and Verizon in different bands, using both standalone (SA) and non-standalone (NSA) modes, as summarized in Table~\ref{tab:indoor_reception}. Indoor Verizon 5G mmWave reception in 28 GHz with a maximum bandwidth of 400 MHz using 4-channel aggregation (CA) was possible in some locations. However, the reception was poor, likely due to the Low-E glass used in the windows. There were only a handful of rooms that were LoS to the BS that could receive 5G mmWave signals when the window was open, as shown in Fig.~\ref{fig:bs_ue_gap}. 
Also, while this particular Verizon BS was capable of transmitting LTE-LAA in the unlicensed 5 GHz band (band 46) and 4G LTE in the Citizens Broadcast Radio Service band (CBRS, band 48), we did not receive transmissions on these bands indoors, even with windows open, most likely due to the lower transmitted power allowed in these bands.

All Verizon 5G NR deployments were NSA, but there was a difference in the LTE primary channel used depending on the NR band. When NR band n5 (low-band, bandwidth 10 MHz) was used, the LTE primary on the DL was always band 66 with a bandwidth of 20 MHz, whereas when NR band n261 (mmWave) was being used, the LTE primary carrier on the DL was either band 66 or band 13 with a bandwidth of 10 MHz. This difference in choice of LTE primary channel has an effect on overall DL and UL throughput as will be explained in the next section. 

==> sections/05.5_discussion.tex <==
\section{Discussion}

The closest recent work on OtI mmWave performance that is comparable to ours is~\cite{kohli2022outdoor}. While both papers deal with the performance of OtI mmWave performance, the methodologies employed are very different, leading to different and contradictory conclusions. Our measurements were specifically conducted on deployed 5G mmWave systems using consumer handsets: thus, all real-world conditions such as beam-management using phased-arrays at both BS and UE, wide-bandwidth operation (400 MHz) and handset limitations are included in the performance we measure. Our performance metrics are direct measurements of throughput (uplink and downlink) and latency. Since these measurements were made on a deployed network, they include all overheads due to the MAC, transport and network layers as well. On the other hand, the throughput results reported in~\cite{kohli2022outdoor} are based on predictions from signal strength measurements using a specific channel sounder that utilizes a continuous-wave tone at 28 GHz as the sounding signal, rotating horn antennas on the receiver and omni-directional transmit antennas: very different from actual operating conditions of 5G mmWave. Further, the effects of the intermediate layers are not accounted for in the prediction. These major differences in measurement methodologies and environment lead to the contradictory results: our results demonstrate that in a building with Low-E glass windows located about 25m from a 5G mmWave BS, there is no 5G mmWave connectivity at all through closed windows and limited connectivity in a few locations with the window open whereas the prediction in~\cite{kohli2022outdoor} is of 1.2 Gbps under similar operating conditions in 90\% of locations. Additionally, our measurements provide comparison of both throughput and latency performance when 5G NR in the low-band is used instead of 5G mmWave and especially in the case of uplink throughput and latency we demonstrate superior performance of the former due to effective aggregation with the LTE primary channel. Further, we compare performance across different bands and operators to demonstrate that OtI performance over 5G mmWave is unavailable in this building when the windows are shut, but low and mid-band 5G NR can provide DL throughput of up to 400 Mbps.


% In this section, we discuss and contrast our results with a recent work. We have demonstrated the performance of outdoor-to-indoor NR in mmWave and low-band, which indicated that in a Low-e windowed building, mmWave connection can only be established under LoS conditions, with low-band channels used as a fail-over in NLoS conditions. A prior work \cite{kohli2022outdoor} has indicated otherwise: using an SNR prediction model that considers a Low-e glass obstacle, the authors predicted the best mmWave performance of at least 1.2 Gbps downlink PHY throughput to 90\% indoor UEs at a distance of up to 25 m using 16-QAM modulation and 1/2 code rate, while at least 0.5 Gbps can be achieved up to 49 m using QPSK 3/10. However, these prediction are modelled based on controlled experiments using a specialized mmWave channel sounder as both BS and UE. In our observation, our smartphone UE cannot connect to a mmWave channel when obstructed by \chk{Low-e window} even with the link distance of \chk{ $\sim$25 m}. Additionally, the prior work only considers PHY layer performance, while we consider application level performance that depends on the in-between layers (\ie MAC, Network, Transport layers) which also influence UE's channel selection.
% In a real-deployment, there are several aspects that affecting channel selection, \eg BS transmit power, RSRP threshold, and beam angle, and we posited that these parameters are different between the real-deployment and controlled experiments. Unfortunately, they are invisible to us due to the black box nature of a commercial BS, thus a new methodology need to be developed to estimate these parameters.


==> sections/05_results_temp.tex <==
\section{Experimental Results}\label{sec:results}

% \begin{figure}[t!]
% \includegraphics[width=0.95\linewidth]{images/001-1-dl.pdf}
% \caption{Downlink throughput performance on all floors.}
% \vspace{-0.3cm}
% \label{fig:dl_tput}
% \end{figure}

% \begin{figure}[t!]
% \includegraphics[width=0.95\linewidth]{images/001-2-ul.pdf}
% \caption{Uplink throughput performance on all floors.}
% \vspace{-0.3cm}
% \label{fig:ul_tput}
% \end{figure}

% \begin{figure}[t!]
% \includegraphics[width=0.95\linewidth]{images/001-3-lat.pdf}
% \caption{Latency performance on all floors.}
% \vspace{-0.3cm}
% \label{fig:latency}
% \end{figure}

% \begin{table}[!t]
% \caption{LoS mmWave Reception (Location A) on Different Floors}
% %\vspace{-0.2cm}
% \centering
% \begin{tabular}{|l|c|c|c|}
% \hline
% \bfseries Floors & \bfseries Beam Index & \bfseries Avg. RSRP & \bfseries Avg. RSRQ \\
% \hline
% \bfseries 2nd (E206) & 4 & -94.17 dBm & -11 dB \\
% \hline
% \bfseries 3rd (E306) & 20 & -98.57 dBm & -11 dB \\
% \hline
% \bfseries 4th (E406) & 20 & -94.36 dBm & -11 dB \\
% \hline
% \bfseries 5th (E506) & 24 & -94.48 dBm & -11 dB \\
% \hline
% \bfseries 6th (E606) & 27 & -103.99 dBm & -11.67 dB \\
% \hline
% \end{tabular}
% \label{tab:mmwave_reception}
% \vspace{-0.5cm}
% \end{table}

\subsection{Performance as a function of floor height}

For this set of experiments, the window in each room was set to the maximum possible opening. As shown in Table~\ref{tab:mmwave_reception}, 5G mmWave signals are received with varying average RSRP levels and different beam indices on floors 2 to 6.
% (2nd to 7th floors), with the exception of the highest 7th floor (at the height of \chk{$\sim 21~m$} from the base of the building). 
When a 5G mmWave connection was available, 4 channel aggregation was always used. We also verified using NSG that all available mmWave RBs were allocated to the UE, indicating that there were no other devices connected to the BS during the experiments. We see from Table~\ref{tab:mmwave_reception} that the average RSRP on the 3rd floor is lower than the 2nd, 4th and 5th floors: this could be due to the beam index not being optimally chosen since we also observe that the beam index (20) was the same for the 3rd and 4th floors.

\begin{table}[!h]
\caption{mmWave at Location A on different floors}
%\vspace{-0.2cm}
\centering
\begin{tabular}{|l|c|c|c|}
\hline
\bfseries Floors & \bfseries Beam Index & \bfseries Avg. RSRP & \bfseries Avg. RSRQ \\
\hline
\bfseries 2nd (E206) & 4 & -94.17 dBm & -11 dB \\
\hline
\bfseries 3rd (E306) & 20 & -98.57 dBm & -11 dB \\
\hline
\bfseries 4th (E406) & 20 & -94.36 dBm & -11 dB \\
\hline
\bfseries 5th (E506) & 24 & -94.48 dBm & -11 dB \\
\hline
\bfseries 6th (E606) & 27 & -103.99 dBm & -11.67 dB \\
\hline
\end{tabular}
\label{tab:mmwave_reception}
\vspace{-0.25cm}
\end{table}

Fig.~\ref{fig:dl_tput} shows the DL throughput performance across the floors, in location A (closest, LoS) to E (farthest, NLoS). In floors 2 - 5, there is a degradation of DL throughput as the UE is moved further inside the room, with the worst DL performance in locations D and E where the UE is no longer connected to 5G mmWave but is instead handed over to low-band NR (band n5 850 MHz, 10 MHz bandwidth). In E606 (6th floor), location B performs better than A: this could be because location A is at the edge of the serving beam, or the wider bandwidth LTE primary on band b66 is being used.

\begin{figure}[t!]
\centering
\includegraphics[width=0.95\linewidth]{images/001-1-dl.pdf}
\caption{Downlink throughput performance on all floors.}
\vspace{-0.3cm}
\label{fig:dl_tput}
\end{figure}

Overall, there is a degradation in DL throughput as the UE is moved to the higher floors as well.
Each floor is served by a different beam index, except for the 3rd and 4th floors. Fig.~\ref{fig:dl_tput} shows a lower DL throughput performance at location B in room E406 (4th floor), compared to the 3rd and 5th floors. This indicates a non-optimal choice of serving beam, \ie the location B of the 4th floor could be a transition area where beam indices 20 and 24 overlap, and the UE may be better served by beam index 24 instead. 

\begin{figure}[t!]
\centering
\includegraphics[width=0.95\linewidth]{images/001-2-ul.pdf}
\caption{Uplink throughput performance on all floors.}
\vspace{-0.3cm}
\label{fig:ul_tput}
\end{figure}

\begin{figure}[t!]
\centering
\includegraphics[width=0.95\linewidth]{images/001-3-lat.pdf}
\caption{Latency performance on all floors.}
\vspace{-0.3cm}
\label{fig:latency}
\end{figure}

Fig.~\ref{fig:ul_tput} shows the UL throughput performance across the floors. Similar to the DL performance, the UL performance of the UE is degraded as the UE is moved to the higher floors, however, the effect of varying location inside a room is not as straightforward. Best UL performance is mostly seen in location A, except for rooms E506 and E606 (5th and 6th floor), respectively. This indicates that a LoS connection to the BS is not enough to guarantee a good UL performance on the higher floors. This could also be due to the fact that the beam at the UE is much wider compared to the BS since there are fewer antenna elements on the UE. Interestingly, when the UE switches to 5G NR low-band in locations D and E in these rooms, the UL throughput improves compared to when connected to 5G mmWave: this could be due to the wider bandwidth (20 MHz) of the LTE primary channel b66 (band 66) in these locations compared to 10 MHz b13 used with 5G mmWave.
Lastly, Fig.~\ref{fig:latency} shows latency performance across the floors, which shows a reverse pattern to the throughput: lower latency values are obtained in locations D and E where the UE is connected to low-band NR and LTE band b66. This indicates that 5G mmWave transmission incurs additional overheads due to beam management requirements, thus leading to increased latency.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=.48\textwidth]{images/gap-diagram.png}
% \caption{Gap measurement diagram.}\label{fig:gap_diagram}
% \vspace{-0.3cm}
% \end{figure}

\subsection{Performance as a function of window opening gap size}

% \begin{table}[!h]
% \caption{NR Reception on Different Gaps}
% %\vspace{-0.2cm}
% \centering
% \begin{tabular}{|l|c|c|c|c|}
% \hline
% \bfseries Gap \# & \bfseries NR Channels & \bfseries Avg. RSRP & \bfseries Avg. RSRQ \\
% \hline
% \bfseries Gap 1 & 4 $\times$ n261 (400 MHz) & -89.52 dBm & -11 dB \\
% \hline
% \bfseries Gap 2 & 4 $\times$ n261 (400 MHz) & -98.98 dBm & -11 dB \\
% \hline
% \bfseries Gap 3 & 1 $\times$ n5 (10 MHz) & -74.34 dBm & -11 dB \\
% \hline
% \bfseries Gap 4 & 1 $\times$ n5 (10 MHz) & -75.60 dBm & -11 dB \\
% \hline
% \end{tabular}
% \label{tab:gap_reception}
% \vspace{-0.5cm}
% \end{table}

% \begin{figure*}[t!]
% \centering
% \begin{subfigure}{.323\textwidth}
%   \includegraphics[width=\textwidth]{images/002-1-dl-gap.pdf}
%   \caption{Downlink throughput.}\label{fig:gap_dl}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.323\textwidth}
%   \includegraphics[width=\textwidth]{images/002-2-ul-gap.pdf}
%   \caption{Uplink throughput.}\label{fig:gap_ul}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.323\textwidth}
%   \includegraphics[width=\textwidth]{images/002-3-lat-gap.pdf}
%   \caption{Round trip latency.}\label{fig:gap_lat}
% \end{subfigure}
% \caption{Throughput and latency performance as a function of window opening size}
% \vspace{-0.3cm}
% \label{fig:gap_perf}
% \end{figure*}

% \begin{figure*}[t!]
% \centering
% \begin{subfigure}{.323\textwidth}
%   \includegraphics[width=\textwidth]{images/004-1-dl-survey-lte.pdf}
%   \caption{LTE downlink throughput.}\label{fig:survey_dl_lte}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.323\textwidth}
%   \includegraphics[width=\textwidth]{images/004-3-ul-survey-lte.pdf}
%   \caption{LTE uplink throughput.}\label{fig:survey_ul_lte}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.323\textwidth}
%   \includegraphics[width=\textwidth]{images/004-5-lat-survey-lte.pdf}
%   \caption{LTE latency.}\label{fig:survey_lat_lte}
% \end{subfigure}
% \\
% \begin{subfigure}{.323\textwidth}
%   \includegraphics[width=\textwidth]{images/004-2-dl-survey-nrnsa.pdf}
%   \caption{NR-NSA downlink throughput.}\label{fig:survey_dl_nrnsa}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.323\textwidth}
%   \includegraphics[width=\textwidth]{images/004-4-ul-survey-nrnsa.pdf}
%   \caption{NR-NSA uplink throughput.}\label{fig:survey_ul_nrnsa}
% \end{subfigure}
% \hfill
% \begin{subfigure}{.323\textwidth}
%   \includegraphics[width=\textwidth]{images/004-6-lat-survey-nrnsa.pdf}
%   \caption{NR-NSA latency.}\label{fig:survey_lat_nrnsa}
% \end{subfigure}
% \caption{Indoor survey of AT\&T, T-Mobile, and Verizon in terms of throughput and latency performance.}
% \vspace{-0.3cm}
% \label{fig:survey_perf}
% \end{figure*}


The best 5G mmWave performance was obtained in room E206 on the 2nd floor. Hence, we performed additional experiments in this room to quantify performance as a function of the window opening gap size. The UE was placed in location A and the width of the window opening was varied as shown in Fig.~\ref{fig:gap_diagram}, where Gap 1 is the widest gap and Gap 4 is a fully closed window. For each gap setting, measurements were taken over 15 minutes.

\begin{figure}[h!]
\centering
\includegraphics[width=.48\textwidth]{images/gap-diagram.png}
\caption{Window opening gap diagram.}\label{fig:gap_diagram}
\vspace{-0.3cm}
\end{figure}

Table~\ref{tab:gap_reception} shows the comparison of UE performance with different gap sizes. For Gap 1 and Gap 2, the UE was connected to mmWave but the RSRP was almost 10 dB lower in the latter case. When the gap was reduced in the Gap 3 and Gap 4 settings, the UE no longer connects to 5G mmWave at all and instead switches to 5G NR in the low-band and there is not much difference in the RSRP since unlike band n261 at 28 GHz, band n5 at 850 MHz propagates very well indoors and is less dependent on the window gap size.





% describes UE's NR reception on different gaps, which shows difference between Gap 1-2 and Gap 3-4 where the UE is connected to mmWave for the former, while for the latter UE is connected to band n5 (low-band NR similar to the prior measurements at location D and E). This difference indicates again, that in this building, outdoor-to-indoor mmWave connection can only be established using LoS.
% Further, we introduced BW-scaled average RSRP in log-scale, namely $B$, to compare RSRP values across different NR channels and bandwidths. The calculation is as follows:
% \begin{equation*}
%     B = (\text{avg. RSRP in dBm}) + 10 \log_{10} (\text{BW in MHz}).
% \end{equation*}
% We observe a steady reduce of $B$ from Gap 1 to 4, even with stable average RSRQ across all gaps. The lowest $B$ achieved in Gap 2 with mmWave connection, further signifying the adverse effect of tightening LoS gap to mmWave signal.

The throughput and latency performance obtained with the various window gap settings are shown by Fig.~\ref{fig:gap_perf}. There is a significant performance difference between Gap 1-2 and Gap 3-4, due to the difference in the NR band being used. The best DL throughput is achieved with the Gap 1 and 2 settings when connected to 5G mmWave as shown by Fig.~\ref{fig:gap_dl}. However, the best UL throughput and latency is achieved by Gap 3 and 4, as shown by Fig.~\ref{fig:gap_ul} and \ref{fig:gap_lat}.
These results agree with the previous results on different floors and corroborate the conclusion that true Gbps throughput over 5G mmWave can only be delivered indoors when there is unobstructed LoS through an open window.

\begin{table}[!h]
\caption{NR Reception on Different Gaps}
%\vspace{-0.2cm}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline
\bfseries Gap \# & \bfseries NR Channels & \bfseries Avg. RSRP & \bfseries Avg. RSRQ \\
\hline
\bfseries Gap 1 & 4 $\times$ n261 (400 MHz) & -89.52 dBm & -11 dB \\
\hline
\bfseries Gap 2 & 4 $\times$ n261 (400 MHz) & -98.98 dBm & -11 dB \\
\hline
\bfseries Gap 3 & 1 $\times$ n5 (10 MHz) & -74.34 dBm & -11 dB \\
\hline
\bfseries Gap 4 & 1 $\times$ n5 (10 MHz) & -75.60 dBm & -11 dB \\
\hline
\end{tabular}
\label{tab:gap_reception}
% \vspace{-0.5cm}
\end{table}

\begin{figure*}[h!]
\centering
\begin{subfigure}{.323\textwidth}
  \includegraphics[width=\textwidth]{images/002-1-dl-gap.pdf}
  \caption{Downlink throughput.}\label{fig:gap_dl}
\end{subfigure}
\hfill
\begin{subfigure}{.323\textwidth}
  \includegraphics[width=\textwidth]{images/002-2-ul-gap.pdf}
  \caption{Uplink throughput.}\label{fig:gap_ul}
\end{subfigure}
\hfill
\begin{subfigure}{.323\textwidth}
  \includegraphics[width=\textwidth]{images/002-3-lat-gap.pdf}
  \caption{Round trip latency.}\label{fig:gap_lat}
\end{subfigure}
\caption{Throughput and latency performance as a function of window opening size}
\vspace{-0.3cm}
\label{fig:gap_perf}
\end{figure*}

\begin{figure*}[h!]
\centering
\begin{subfigure}{.323\textwidth}
  \includegraphics[width=\textwidth]{images/004-1-dl-survey-lte.pdf}
  \caption{LTE downlink throughput.}\label{fig:survey_dl_lte}
\end{subfigure}
\hfill
\begin{subfigure}{.323\textwidth}
  \includegraphics[width=\textwidth]{images/004-3-ul-survey-lte.pdf}
  \caption{LTE uplink throughput.}\label{fig:survey_ul_lte}
\end{subfigure}
\hfill
\begin{subfigure}{.323\textwidth}
  \includegraphics[width=\textwidth]{images/004-5-lat-survey-lte.pdf}
  \caption{LTE latency.}\label{fig:survey_lat_lte}
\end{subfigure}
\\
\begin{subfigure}{.323\textwidth}
  \includegraphics[width=\textwidth]{images/004-2-dl-survey-nrnsa.pdf}
  \caption{NR-NSA downlink throughput.}\label{fig:survey_dl_nrnsa}
\end{subfigure}
\hfill
\begin{subfigure}{.323\textwidth}
  \includegraphics[width=\textwidth]{images/004-4-ul-survey-nrnsa.pdf}
  \caption{NR-NSA uplink throughput.}\label{fig:survey_ul_nrnsa}
\end{subfigure}
\hfill
\begin{subfigure}{.323\textwidth}
  \includegraphics[width=\textwidth]{images/004-6-lat-survey-nrnsa.pdf}
  \caption{NR-NSA latency.}\label{fig:survey_lat_nrnsa}
\end{subfigure}
\caption{Indoor survey of AT\&T, T-Mobile, and Verizon in terms of throughput and latency performance.}
\vspace{-0.3cm}
\label{fig:survey_perf}
\end{figure*}

% and the prior location-based measurement results further show a great downlink throughput performance by mmWave, which is also greatly limited by LoS connection and range. On the other hand, the mmWave connection is performing lesser on uplink throughput and latency compared low-band NR.

\subsection{Comparison of 5G NR performance among different bands and operators}
We surveyed floors 2 - 7 of the building using three identical Google Pixel 5 phones, one for each operator. The phones were placed on a cart and wheeled to different rooms in the building facing the mmWave BS, not just the ones where the detailed measurements were performed. Measurements were taken in corridors as well. All windows were shut during this survey. As stated previously, Verizon 5G mmWave was not received at all on the 7th floor, but other bands and operators were, so the results presented in Fig.~\ref{fig:survey_perf} include measurements on the 7th floor. {\it Since all windows were shut, no Verizon 5G mmWave was received even in rooms directly facing the mmWave BS.} We also confirmed from our measurements that all Verizon channels in all NR and LTE bands that were received inside the building were being transmitted from the BS on the pole right outside the building. However, we are uncertain about the exact location of the AT\&T and T-Mobile BSs.

\noindent \textbf{DL Throughput comparison:} From Figs.~\ref{fig:survey_dl_lte} and ~\ref{fig:survey_dl_nrnsa} we see that NR clearly delivers significant DL throughput improvements over LTE, especially for T-Mobile and Verizon. AT\&T NR performance is limited due to the low-band only deployment using only 5 MHz of bandwidth, compared to T-Mobile's 100 MHz at 2.5 GHz and Verizon's 10 MHz. Since Verizon 5G mmwave was not received during these tests, the DL throughput is solely via aggregation of LTE and low-band NR. With no mmWave reception, T-Mobile NR DL throughput is superior to Verizon's, even though the Verizon BS is very close to the building. Once again, this survey demonstrates the severe limitation of indoor 5G mmWave reception. 

\noindent \textbf{UL Throughput comparison:} From Figs.~\ref{fig:survey_ul_lte} and ~\ref{fig:survey_ul_nrnsa} we see that here too NR clearly delivers significant UL throughput improvements over LTE, for all operators. There is a clear advantage of Verizon UL, most likely due to the aggregation with the 20 MHz band 66 LTE carrier and the proximity of the location to the BS enabling higher modulation-coding settings. For example, the 80 Mbps throughput is due to 65 Mbps over band 66 and only 15 Mbps over NR band n5.

\noindent \textbf{Latency comparison:} From Figs.~\ref{fig:survey_lat_lte} and ~\ref{fig:survey_lat_nrnsa} we see that there is not an appreciable reduction in latency with NR, though overall Verizon latency with NR is the lowest. However previous results already noted that NR latency was lower in the low-band compared to mmWave, and these results only include low-band NR. It should also be noted that since most of these measurements were over the NSA mode of NR, the latency could be higher due to the dual connectivity, channel aggregation and the use of the 4G core network. As SA with the new 5G core begins to be deployed, we anticipate that the latency results will improve.



% \begin{figure}[t!]
% \includegraphics[width=0.95\linewidth]{images/003-1-dl.pdf}
% \caption{Average downlink throughput performance on all floors.}
% \vspace{-0.3cm}
% \label{fig:dl_tput}
% \end{figure}

% \begin{figure}[t!]
% \includegraphics[width=0.95\linewidth]{images/003-2-ul.pdf}
% \caption{Average uplink throughput performance on all floors.}
% \vspace{-0.3cm}
% \label{fig:ul_tput}
% \end{figure}

% \begin{figure}[t!]
% \includegraphics[width=0.95\linewidth]{images/003-3-lat.pdf}
% \caption{Average latency performance on all floors.}
% \vspace{-0.3cm}
% \label{fig:latency}
% \end{figure}
